Variable stars in the globular cluster NGC 7492. New discoveries and physical parameters determination

We have performed a photometric V, R, I CCD time-series analysis with a baseline of ~8 years of the outer-halo globular cluster NGC 7492 with the aim of searching for new variables and using these (and the previously known variables) to determine the physical parameters of interest for the cluster (e.g. metallicity, absolute magnitude of the horizontal branch, distance, etc.). We use difference image analysis (DIA) to extract precise light curves in the relatively crowded star field, especially towards the densely populated central region. Several approaches are used for variability detection that recover the known variables and lead to new discoveries. We determine the physical parameters of the only RR0 star using light curve Fourier decomposition analysis. We find one new long period variable and two SX Phe stars in the blue straggler region. We also present one candidate SX Phe star which requires follow-up observations. Assuming that the SX Phe stars are cluster members and using the period-luminosity relation for these stars, we estimate their distances as ~25.2+-1.8 and 26.8+-1.8 kpc, and identify their possible modes of oscillation. We refine the periods of the two RR Lyrae stars in our field of view. We find that the RR1 star V2 is undergoing a period change and possibly exhibits the Blazhko effect. Fourier decomposition of the light curve of the RR0 star V1 allows us to estimate the metallicity [Fe/H]_ZW-1.68+-0.10 or [Fe/H]_UVES-1.64+-0.13, log-luminosity ~1.76+-0.02, absolute magnitude ~0.38+-0.04 mag, and true distance modulus of ~16.93+-0.04 mag, which is equivalent to a distance of ~24.3+-0.5 kpc. All of these values are consistent with previous estimates in the literature.

==> aa.tex <==
\BeginSolutions
\EndSolutions

